NOVIS: A Case for End-to-End Near-Online Video Instance Segmentation

Until recently, the Video Instance Segmentation (VIS) community operated under the common belief that offline methods are generally superior to a frame by frame online processing. However, the recent success of online methods questions this belief, in particular, for challenging and long video sequences. We understand this work as a rebuttal of those recent observations and an appeal to the community to focus on dedicated near-online VIS approaches. To support our argument, we present a detailed analysis on different processing paradigms and the new end-to-end trainable NOVIS (Near-Online Video Instance Segmentation) method. Our transformer-based model directly predicts spatio-temporal mask volumes for clips of frames and performs instance tracking between clips via overlap embeddings. NOVIS represents the first near-online VIS approach which avoids any handcrafted tracking heuristics. We outperform all existing VIS methods by large margins and provide new state-of-the-art results on both YouTube-VIS (2019/2021) and the OVIS benchmarks.

==> figures/qualitative_results_failure_cases.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.24\textwidth]{figures/qualitative_results/ytvis_19_21/0a49f5265b/00000.jpg}
    \includegraphics[width=0.24\textwidth]{figures/qualitative_results/ytvis_19_21/0a49f5265b/00030.jpg}
    \includegraphics[width=0.24\textwidth]{figures/qualitative_results/ytvis_19_21/0a49f5265b/00060.jpg}
    \includegraphics[width=0.24\textwidth]{figures/qualitative_results/ytvis_19_21/0a49f5265b/00090.jpg}    
    \caption{
    %
    Example \textbf{failure cases} from any of the presented VIS benchmark validation sets.
    %
    We show outputs from our ~\method{} model with the top-performing Swin-L~\cite{SwinTransformer} backbone.
    %
    }
    \label{fig:qualitative_results_failure_cases}
\end{figure*}
